ThingPot: an interactive Internet-of-Things honeypot

The Mirai Distributed Denial-of-Service (DDoS) attack exploited security vulnerabilities of Internet-of-Things (IoT) devices and thereby clearly signalled that attackers have IoT on their radar. Securing IoT is therefore imperative, but in order to do so it is crucial to understand the strategies of such attackers. For that purpose, in this paper, a novel IoT honeypot called ThingPot is proposed and deployed. Honeypot technology mimics devices that might be exploited by attackers and logs their behavior to detect and analyze the used attack vectors. ThingPot is the first of its kind, since it focuses not only on the IoT application protocols themselves, but on the whole IoT platform. A Proof-of-Concept is implemented with XMPP and a REST API, to mimic a Philips Hue smart lighting system. ThingPot has been deployed for 1.5 months and through the captured data we have found five types of attacks and attack vectors against smart devices. The ThingPot source code is made available as open source.

==> title.tex <==
\begin{titlepage}


\begin{center}

%% Insert the TU Delft logo at the bottom of the page.

%% Print the title in cyan.
{\makeatletter
\largetitlestyle\fontsize{84}{114}\selectfont\@title
%\largetitlestyle\color{tudelft-cyan}\Huge\@title
\makeatother}

%% Print the optional subtitle in black.
{\makeatletter
\ifx\@subtitle\undefined\else
    \bigskip
   {\tudsffamily\fontsize{42}{62}\selectfont\@subtitle}    
    %\titlefont\titleshape\LARGE\@subtitle
\fi
\makeatother}

\bigskip
\bigskip

by
%door

\bigskip
\bigskip

%% Print the name of the author.
{\makeatletter
%\largetitlefont\Large\bfseries\@author
\largetitlestyle\fontsize{26}{26}\selectfont\@author
\makeatother}

\bigskip
\bigskip

to obtain the degree of Master of Science
%ter verkrijging van de graad van Master of Science

at the Delft University of Technology,
%aan de Technische Universiteit Delft,

to be defended publicly on Tuesday August 29, 2017 at 13:30.\\
%in het openbaar de verdedigen op dinsdag 1 januari om 10:00 uur.
\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip
\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip
\begin{tabular}{lll}
    Student number: & 4502663 \\
    Project duration: & \multicolumn{2}{l}{November 27th, 2016 -- August 29th, 2017} \\
    Thesis committee: &  Dr.\ ir.\ Fernando \ A.\ Kuipers & TU Delft, supervisor \\
        & Marco Zuniga, PhD & TU Delft \\
        & Ir.\ Javier Santillan, & Brightsight B.V. , supervisor
\end{tabular}
\bigskip
\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip
\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip\bigskip
%\emph{Op dit verslag is geheimhouding van toepassing tot en met 31 december 2013.}
\bigskip
\\
An electronic version of this thesis is available at \url{http://repository.tudelft.nl/}.
%\\[1cm]

%\centering{\includegraphics{cover/logo_black}}


\end{center}

\begin{tikzpicture}[remember picture, overlay]
    \node at (5,-2)[anchor=south,inner sep=0pt]{
        \includegraphics{cover/logo_black}
    };
    % \node at (current page.south)[anchor=south,inner 
    \node at (10,-1.4)[anchor=south,inner
    sep=0pt]{
        \includegraphics[width=0.2\linewidth]{brslogo.png}
    };
\end{tikzpicture}

\end{titlepage}


